Optimizing Sensing Matrices for Spherical Near-Field Antenna Measurements

In this article, we address the problem of reducing the number of required samples for Spherical Near-Field Antenna Measurements (SNF) by using Compressed Sensing (CS). A condition to ensure the numerical performance of sparse recovery algorithms is the design of a sensing matrix with low mutual coherence. Without fixing any part of the sampling pattern, we propose sampling points that minimize the mutual coherence of the respective sensing matrix by using augmented Lagrangian method. Numerical experiments show that the proposed sampling scheme yields a higher recovery success in terms of phase transition diagram when compared to other known sampling patterns, such as the spiral and Hammersley sampling schemes. Furthermore, we also demonstrate that the application of CS with an optimized sensing matrix requires fewer samples than classical approaches to reconstruct the Spherical Mode Coefficients (SMCs) and far-field pattern.

==> Sections/acknowledgement.tex <==
\section{Acknowledgement}
The authors would like to thank Arash Behboodi for many fruitful discussions on the topics
addressed in the present paper

==> Sections/conclusions.tex <==
\section{Conclusions}\label{sec7_conclusion}
We have discussed the methods to optimize sensing matrices for the \ac{CS}-based \ac{SNF} method. In contrast to the conventional method, which requires an oversampled near-field measurement, the \ac{CS}-based method can significantly reduce the number of samples to reconstruct the far-field pattern by using an optimized sensing matrix. The strategy emanates from the fact that, in most cases, the \ac{SMCs} are compressible. Harnessing this information is key in implementing the \ac{CS}-based method.

We propose two different approaches, namely gradient-based and \ac{ALM} based proximal methods, to design low coherence sensing matrices that are suitable for the \ac{CS}-based method. Numerical experiments show that these approaches are successful in minimizing the coherence of sensing matrices constructed from Wigner D-functions and spherical harmonics. Numerical simulations from measurement data show that the proposed sampling schemes can reconstruct the far-field pattern with a reasonable error while reducing the number of sampling points. Additionally, numerical experiments show that the optimization methods maintain the uniformity structure of proposed sampling points, hence making it easier to implement in real measurement system.


==> Sections/cs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Compressed Sensing}\label{sec2_cs}
%\textcolor{blue}{Arya, a big part of this section is used also in our other papers. Make sure you change it adequately so it is not plagiarism.}

In most signal acquisition processes, it is enough to model the {measurement processes} with a linear system as follows:
\begin{equation}
\label{eq:linear_meas}
    \mbf y = \mbf A \mbf x,
\end{equation}
where $\mbf A \in \C^{K \times L}$ is the sensing matrix. \ac{CS} provides a framework to recover the sparse structure of $\mbf{x}$ from a smaller dimension of the acquired signal $\mbf y \in \C^K$, i.e., $K < L$. {\acf{BP} is one of the well-known algorithms to estimate the sparse vector $\mbf{x}$ by solving the following optimization problem}
\begin{equation}
\tag{P1}\label{ch2:eq P1}
\begin{aligned}
& \underset{\mbf{\hat x}}{\text{minimize}}
& & \norm{\mathbf{\hat x}}_1
& \text{subject to}
& & \mbf y = \mbf A \mbf{\hat x}.
\end{aligned}
\end{equation}
Theoretically speaking, it is necessary to have a fundamental limit on the required number of measurements $K$ to ensure the unique reconstruction of sparse vector $\mbf x$, meaning that the estimated vector $\mbf{\hat x}$ and the ground truth vector $\mbf{x}$ are close enough in terms of small numerical differences. Low coherence of the matrix $\mbf A$ are well-known properties to provide a sufficient condition and robustness of the reconstruction of sparse vector $\mbf{x}$ \cite{gribonval2003sparse,candes2005decoding,candes2006robust}.

For a matrix $\mbf A=[\vec{a}_1 \dots \vec{a}_L]\in\mbb C^{K \times L}$, the {\color{black}mutual} coherence is defined as
\[
 \mu
 (\mbf{A})\defeq\max_{1\leq i<j\leq L}\frac{\card{\langle\vec{a}_i,\vec{a}_j\rangle}}{\norm{\vec{a}_i}_2  \norm{\vec{a}_j}_2},
\]
where the lowest coherence we can get is lower bounded by the Welch bound \cite{welch_lower_1974}, which is given as
$$
\mu(\mbf A) \geq \sqrt{\frac{L - K }{K(L-1)}}.
$$
\begin{comment}
Taking this bound with the number of sparsity $s$, the recovery guarantee by using \ac{BP} in \eqref{ch2:eq P1} is achieved when the number of samples $K \gtrsim s^2$, which is sub-optimal because the number of measurements scales in terms of quadratic sparsity order.}

\ABCor{The measurement bound can be improved by considering the \ac{RIP} of a matrix $\mbf{A}$, where for all sparse vectors $\mbf x$ it should satisfy
$$
(1-\delta)\leq \frac{\norm{\mathbf{Ax}}_2^2}{\norm{\mathbf x}_2^2}\leq (1+\delta),
$$
for $\delta \in (0,1)$. If a certain matrix $\mbf A$ satisfies this property, then the number of samples is given by $K \gtrsim s\log(L)$, which now improves the measurement bound scaled linearly with the sparsity order $s$. A vast amount of research has been done since then to construct sensing matrices that satisfy the \ac{RIP} condition, specifically for a class of random matrices \cite{rudelson2008sparse, foucart2013mathematical}. Despite remarkable results and theory for random matrices that fulfill the \ac{RIP}, the construction in the deterministic setting is challenging in general   \cite{bandeira2013certifying,tillmann2014computational}.}
\end{comment}
Nonetheless, constructing a low coherence sensing matrix is generally considered important for practical purposes. Before discussing the construction of the sensing matrix for \ac{SNF}, the next section will cover the measurement setting {\color{black}and the mathematical framework of} \ac{SNF}.
\begin{comment}
 The key insight of \ac{CS} relies on the structure of the matrix $\mbf A$ and the reconstruction algorithms to recover the sparse vector $\mbf x$.
\todo[inline]{Changing the next two sentences. They read weird} The structure of matrix $\mbf A$ plays an essential role in guaranteeing a unique reconstruction, at least in theory. The recovery of the sparse vector $\mbf x$ can be done with \ac{BP} \cite{candes2005decoding,rudelson2008sparse}, as described by
\begin{equation}
\tag{P1}\label{ch2:eq P1}
\begin{aligned}
& \underset{\mbf x}{\text{minimize}}
& & \norm{\mathbf{x}}_1
& \text{subject to}
& & \mbf y = \mbf A \mbf x.
\end{aligned}
\end{equation}
In the seminal work of \ac{CS} \cite{candes2005decoding,candes2006robust}, the \ac{RIP} is used to provide a sufficient condition and robustness of the reconstruction against a noisy signal as described by
$$
(1-\delta)\norm{\mathbf x}_2^2\leq \norm{\mathbf{Ax}}_2^2\leq (1+\delta)\norm{\mathbf x}_2^2. 
$$
A vast amount of research has been done since then to construct sensing matrices that satisfy the \ac{RIP} condition, specifically for a class of random matrices \cite{rudelson2008sparse, foucart2013mathematical}. Despite remarkable results and theory for random matrices that fulfil \ac{RIP}, the construction in the deterministic setting is challenging in general   \cite{bandeira2013certifying,tillmann2014computational}. 

Another metric commonly used to design a sensing matrix is the coherence.  For a matrix $\mbf A=[\vec{a}_1 \dots \vec{a}_L]\in\mbb C^{K \times L}$, the {\color{red}mutual} coherence is defined as
\[
 \mu
 (\mbf{A})\defeq\max_{1\leq i<j\leq L}\frac{\card{\langle\vec{a}_i,\vec{a}_j\rangle}}{\norm{\vec{a}_i}_2  \norm{\vec{a}_j}_2}.
\]
At its core, the coherence measures the similarity between normalized adjacent columns of a matrix, and the lowest coherence we can get is bounded by the so-called Welch bound \cite{welch_lower_1974}, which is given as
$$
\mu(\mbf A) \geq \sqrt{\frac{L - K }{K(L-1)}}.
$$
It is desirable to design a matrix that achieves the Welch bound to attain a better{\color{red}, if not the best,} sparse recovery performance {\color{red}from a defined number of samples} \cite{gribonval2003sparse,donoho2005stable}. Although it generates a sub-optimal measurement bound to recover the sparse signal, \todo[inline]{why? what does a sub-optimal measurement bound mean?} in terms of squared sparsity, \todo[inline]{why in terms of squared sparsity? What does that mean?} the coherence is easy to compute and can be used to design a deterministic sensing matrix for practical purposes. Before discussing the construction of the sensing matrix for \ac{SNF}, in the next section, we will discuss the measurement setting {\color{red}and the mathematical framework of} \ac{SNF}.
\end{comment}

==> Sections/exp_cohsparse.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical Evaluation}
\label{sec5_NumEval}
In this section, we perform the numerical optimization of the sensing matrix for general construction as discussed in Section \ref{Sec:General}, as well as in Section \ref{Sec:Specific}.
%, as discussed as well in \cite[Sec. 4.4]{hansen1988spherical}
%including Wigner D-functions and spherical harmonics, and the specific case for linearly polarized probe in Section \ref{Sec:Specific}, as discussed as well in \cite[Sec. 4.4]{hansen1988spherical}. 
The sampling points from the gradient-based Algorithm \ref{algo_gd}, as well as the \ac{ALM}-based Algorithm \ref{algo_ALM}, are compared to two known sampling patterns: the spiral \cite{saff1997distributing} and the Hammersley \cite{cui1997equidistribution} sampling pattern. For all cases, we do sparse recovery by using YALL1 \cite{yang2011alternating}. The results show the average of $100$ sparse-recovery trials with randomly sparse \ac{SMCs} generated following a zero-mean, unit-variance Gaussian distribution.
\begin{comment}
\subsection{Evaluating $\ell_p$-norm}
Since we approximate the $\ell_\infty$-norm by using the $\ell_p$-norm for a high enough $p \in [2,\infty)$, we present the coherence evaluation for different values of $p$ as depicted in Fig.~\ref{Fig_p_norm} for both spherical harmonics and Wigner D-functions in general setting. 
\begin{figure}[!htb]
\centering
\inputTikZ{0.5}{Figure/Evaluate_p_norm.tex} 
\caption{Coherence of (a) spherical harmonics ($L = 99$) and (b) Wigner D-functions ($L = 83$) sensing matrix with respect to $\ell_p$-norm}
\label{Fig_p_norm}
\end{figure}  
Increasing $p$ can improve coherence minimization. However, starting from $p \geq 4$, the coherence cannot be improved significantly. The same phenomenon can be observed when we increase the number of samples, therby providing the rule of thumb of choosing the value of $p$ when implementing the algorithm. 
\end{comment}
\subsection{General Case}
In the general case, the whole range of orders $-n \leq \mu,m \leq n$ is considered. Hence, the sensing matrix is simply given by the expansion of all degrees and orders, as in \eqref{sec3_expand}. For spherical harmonics, the matrix can be derived directly by setting $\mu = 0$ as introduced in \eqref{eq.sh_wign}.
\subsubsection{Wigner D-functions}
The numerical coherence for a sensing matrix from Wigner D-functions when all angles are optimized is given in Fig.~\ref{Fig_Wigner_uniform}, where in this case, we evaluate $N = 3$ with column dimension $L = 83$. Since our algorithms are initialized randomly, the shown coherence is an average of the results, presented together with their deviation.
\begin{figure}[!htb]
\centering
%\inputTikZ{0.7}{Figure/wigner_admm_gd.tex} 
\inputTikZ{0.55}{Figure/coherence_wigner.tex} 
\caption{Coherence of Wigner D-functions sensing matrix}
\label{Fig_Wigner_uniform}
\end{figure}
For the spiral and Hammersley sampling schemes, the samples along the polarization angle are distributed evenly within the interval $\chi \in [0,2\pi)$. It can be seen that these sampling points generate the worst coherence compared to the sampling points produced by considering the gradient method and \ac{ALM}, described in Algorithm \ref{algo_gd} and \ref{algo_ALM}. Furthermore, the performance of optimized sensing matrices in terms of sparse recovery by using a phase transition diagram is presented in Fig.~\ref{Fig_pt_wigner} . In contrast to the spiral and Hammersley samplings, that yield a high coherence sensing matrix, the optimized sampling points using the gradient descent and \ac{ALM} deliver a better recovery and performance similar to the random sampling's. The graphs depict the transition bounds at a $50\%$ success of recovery with \ac{BP} as in \eqref{ch2:eq P1}. The bounds are tight, so that probability of success is $100\%$ almost immediately below the curve, while it is $0\%$ almost immediately above the curve. The abscissa shows $(K/L)$, that is, the number of samples $K$ with respect to the total number of unknowns $L$, while the ordinate shows the ratio between the sparsity of the vector $\tilde{s}$ and the number of samples acquired $K$. 
\begin{figure}[!htb]
\centering
%\inputTikZ{0.7}{Figure/pt_wigner_admm_gd.tex} 
\inputTikZ{0.55}{Figure/pt_wigner_alm_gd.tex} 
\caption{Phase transition diagram for the sparse recovery with Wigner D-functions, general case.}
\label{Fig_pt_wigner}
\end{figure}  
\subsubsection{Spherical harmonics}
 The main difference with the Wigner D case is the lack of polarization angle $\chi \in [0,2\pi)$. Thereby, we only optimize the elevation $\theta$ and azimuth $\phi$ angles. The average coherence of a sensing matrix constructed with spherical harmonics with $N = 9$ and column dimension of the matrix $L = 99$ is shown in Fig.~\ref{Fig_SH_uniform}.
\begin{figure}[!htb]
\centering
%\inputTikZ{0.7}{Figure/sh_admm_gd.tex} 
\inputTikZ{0.55}{Figure/coherence_sh.tex} 
\caption{Coherence of sensing matrices from spherical harmonics.}
\label{Fig_SH_uniform}
\end{figure}
Similar to the results shown for Wigner D-functions, the optimized sampling points yield a lower-coherence sensing matrix for the spherical harmonics case compared to the construction from spiral and Hammersley schemes. Additionally, optimizing the sampling both on elevation $\theta$ and azimuth $\phi$ yields a lower coherence compared to the theoretical bound, as discussed in \cite{bangun_sensing_2020, bangun2021tight}, at least numerically. 

Fig.~\ref{fig.sphere_dist} shows the distribution of the optimized sampling points on the sphere for the spherical harmonics case. The distribution follows a specific pattern that is approximately equidistant on a geodesic, which demonstrates uniformity of the optimized sampling points.

\begin{figure}[!htb]
\centering
\includegraphics[scale=0.45]{Figure/sampling_new.pdf}
\caption{Sampling distribution from an optimized sensing matrix from spherical harmonics. (a) \ac{ALM} $\left(K = 97 , N = 9 \right)$ (b) Grad. Descent $\left(K =  97  , N = 9 \right)$ (c) $\ac{ALM} \left(K =  400 , N =  21  \right)$ (d) Grad. Descent $\left(K =  400 , N =  21 \right)$}
\label{fig.sphere_dist}
\end{figure}
The phase transition diagram is depicted in Fig.~\ref{Fig_pt_sh}. It can be seen that the optimized sensing matrix yields a performance similar to the random sampling's, and shows a better recovery compared to the spiral and Hammersley samplings. 
\begin{figure}[!htb]
\centering
%\inputTikZ{0.7}{Figure/pt_sh_admm_gd.tex} 
\inputTikZ{0.55}{Figure/pt_sh_alm_gd.tex} 
\caption{Phase transition diagram for sparse recovery of spherical harmonics.}
\label{Fig_pt_sh}
\end{figure}  
\subsection{Specific Case: Practical SNF Measurements}
In most cases, we only evaluate the order $\mu = \pm 1$ with linearly polarized probes for polarization angles $\chi = 0$ and $\chi = \frac{\pi}{2}$. This condition is not contrived and has practical relevance, as discussed in \cite{hansen1988spherical, wacker1975non}. In addition, we can provide experimental data from real measurements, which makes this case even more interesting, as explained in Section \ref{Sec:Specific}. Additionally, in this section we perform the far-field reconstruction with fewer sampling points, i.e., $K < L$, compared to the conventional settings that require a total of $K > 2L$ measurements.
\begin{figure}[!htb]
\centering
%\inputTikZ{0.7}{Figure/snf_admm_gd.tex} 
\inputTikZ{0.55}{Figure/coherence_snf.tex} 
\caption{Coherence of sensing matrices for practical \ac{SNF} measurements.}
\label{Fig_snf_uniform}
\end{figure} 

Since we only consider $\mu = \pm 1$ and polarization angles $\chi = 0$ and $\chi = \frac{\pi}{2}$, we only optimize the elevation $\theta $ and azimuth $\phi$ angles. Fig.~\ref{Fig_snf_uniform} presents the coherence of the sensing matrix from a specific setting constructed from several sampling points. The difference between this specific case compared to the general case in the previous section is that our sensing matrix results from concatenating the matrix constructed from Wigner D-functions for both values of $\chi$ considered, as derived in \eqref{sec3_expand2}. The optimized sensing matrix, again, produces lower coherence compared to known deterministic sampling schemes. 

\begin{figure}[!htb]
\centering
%\inputTikZ{0.7}{Figure/pt_snf_admm_gd.tex} 
\inputTikZ{0.6}{Figure/pt_snf_alm_gd.tex} 
\caption{Phase transition diagram for sparse recovery for practical \ac{SNF} measurements.}
\label{Fig_pt_snf}
\end{figure}  

Furthermore, the optimized sensing matrix also shows higher recovery chances than the spiral and Hammersley sampling schemes, as depicted in Fig.~\ref{Fig_pt_snf}. Moreover, compared to random sampling points with arbitrary polarization angles $\chi$, the optimized sampling points deliver a similar performance while keeping the polarization angles alternate between $\chi = 0$ and $\chi = \frac{\pi}{2}$.


==> Sections/exp_farfield.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Reconstruction of the Far Field}\label{sec6_farfield}
To highlight the potential practical relevance of our proposed sampling scheme, we apply the optimized sampling points in the experimental setting of SNF measurement with a cavity-backed bowtie antenna, with $N = 16$ and, thus, a column dimension of the sensing matrix $L = 576$. The original measurement is acquired through equiangular sampling using a linearly polarized probe and an angular resolution $\Delta\theta = \Delta \phi = 10^{\circ}$. The measurement frequency is $f = 2.4$ GHz. In addition, the results are compared to the conventional method's, where the number of samples required is at least $K > 2L$ \cite{hansen1988spherical}. The SMCs calculated in the classical way are used to generate the points of our proposed sampling by direct application of \eqref{sec3_trans_eq}. These points represent a simulation of a measurement, i.e., the reconstruction of the sampled values from measurement data, and are used for the remaining reconstruction.

\begin{figure}[!htb]
\centering
\inputTikZ{0.4}{Figure/PatternBothPhi0.tex} 
\caption{Far-field reconstruction using optimized sampling points from (a) \ac{ALM}, (b) Gradient Descent $(\phi$-cut $= 0 )$}
\label{Fig_both_farfield_pattern}
\end{figure}  
First, we estimate the \ac{SMCs} by solving an underdetermined system of linear equations, as described in \eqref{sec3_expand2}, by using \ac{BP} as in \eqref{ch2:eq P1}. The sensing matrix is constructed with optimized sampling points that yield low coherence as presented in Fig.~\ref{Fig_snf_uniform}. Specifically, we choose the numbers of samples $K = 242, 422$, which are smaller than the minimum samples required by using the conventional method. Second, we use the estimated \ac{SMCs} to get the far-field pattern and observe the differences in the reconstruction by using the conventional method for linearly polarized probes, i.e., considering only $\mu = \pm 1$ modes \cite{hansen1988spherical}.
\begin{figure}[!htb]
\centering
\inputTikZ{0.4}{Figure/PatternErrorBoth.tex} 
\caption{Maximum and mean error of far-field reconstructions using optimized sampling points from (a) \ac{ALM}, (b) Gradient Descent.}
\label{Fig_both_error_pattern}
\end{figure}  
Fig.~\ref{Fig_both_farfield_pattern} shows a comparison between the ground truth, the far-field pattern calculated from the original measurement, and the reconstruction using \ac{CS} with optimized sensing matrices from Algorithm \ref{algo_gd} and \ref{algo_ALM}. The main cut $\phi = {0}^{\circ}$ is shown. For both cases, it can be seen that the reconstruction is possible with fewer measurement points by using \ac{CS}. In addition, increasing the number of measurements from $K = 242$ to $K = 422$ could improve the accuracy of the reconstruction up to $5$ dB, as seen in Fig.~\ref{Fig_both_error_pattern}, where the numerical evaluation of the maximum and mean errors of the far-field reconstructions are presented.
\begin{comment}
\begin{itemize}
	\item Image antenna?
    \item Explain the antenna under test and its parameters ( B, etc)
    \item Show the reconstruction of 3D, reconstruction of slices?
    \item Error reconstruction of the far-field compared to classical approach vs reduced number measurement
\end{itemize}


\begin{figure}[!htb]
\centering
\inputTikZ{0.7}{Figure/PatternBFDiP002_ADMMPhi0.tex} 
\caption{Far-field reconstruction using optimized sampling points from \ref{algo_ALM} $(\phi$-cut $= 0 )$}
\label{Fig_admm_phicut}
\end{figure}   

\begin{figure}[!htb]
\centering
\inputTikZ{0.7}{Figure/PatternBFDiP002_GDPhi0.tex} 
\caption{Far-field reconstruction using optimized sampling points from \ref{algo_gd} $(\phi$-cut $= 0)$}
\label{Fig_gd_phicut}
\end{figure}  
\begin{figure}[!htb]
\centering
\inputTikZ{0.7}{Figure/ErrorComparisonBFDiP002_ADMM.tex} 
\caption{Error ADMM}
\label{Fig_admm_error}
\end{figure}  

\begin{figure}[!htb]
\centering
\inputTikZ{0.7}{Figure/PatternErrorComparisonBFDiP002_ADMM.tex} 
\caption{ Error ADMM}
\label{Fig_admm_error_pattern}
\end{figure}  


  
\begin{figure}[!htb]
\centering
\inputTikZ{0.7}{Figure/ErrorComparisonBFDiP002_GD.tex} 
\caption{Error GD}
\label{Fig_gd_error}
\end{figure}  

\begin{figure}[!htb]
\centering
\inputTikZ{0.7}{Figure/PatternErrorComparisonBFDiP002_GD.tex} 
\caption{ Error GD}
\label{Fig_gd_error_pattern}
\end{figure}  
\end{comment} 

==> Sections/introduction.tex <==
\section{Introduction}\label{sec1_intro}
Compared to other acquisition methods to characterize an antenna's radiation pattern, \acf{SNF} are a convenient and cost-effective way of ascertaining the radiation characteristics of an \ac{AUT}. {\color{black} Additionally, since the measurement conditions in smaller ranges are easier to control and the obtained results undergo a mathematical transformation that forces them to be physical, their accuracy is higher than for other methods, going as far as being considered the most accurate antenna measurement method \cite{Breinbjerg2016SNF}}. While the biggest challenge of this method may seem the implementation of the mathematical \ac{NFFFT}, one of the most challenging problems is, in fact, the choice of the measurement's sampling strategy. The chosen sampling strategy must ensure that the information of interest is included from an information-theory standpoint and must, also, enable a convenient \ac{NFFFT}. Classically, the Nyquist theorem is applied to the equator of the \ac{AUT} to derive the angular resolution of the sampling scheme, and this angular step is replicated for both classical sampling axes -- azimuth and elevation. The resulting sampling scheme is often called equiangular, and its main drawback is that, considering an information-theory perspective, it results in an equation system with more than double the number of equations, i.e., samples, than variables, i.e., \acf{SMCs} \cite{hansen1988spherical}. As a consequence, one of the strongest objections to this method is its long acquisition time. 

Vibrant research activity has been done to overcome this issue. 
\textcolor{black}{
For instance, the authors of \cite{bucci2001new} use a spiral scanning approach to reduce the density of the samples near the spherical poles, which is a direct implication of using an equiangular sampling.}
Along the same lines, the strategy to reduce sampling points on azimuthal axes has been proposed in \cite{varela2020under}. In addition, the authors also provide an aliasing error estimator to address the aliasing problem that appears naturally when reducing the samples on these axes.
% For instance, by reducing the number of samples using different sampling schemes, as discussed in \cite{bucci2001new}, where the authors use a spiral scanning approach to reduce the density of the samples that towards the spherical poles, which is a direct implication of using an equiangular sampling. Along the same lines, the strategy to reduce sampling points on azimuthal axes has been proposed in \cite{varela2020under}. In addition, the authors also provide an aliasing error estimator to address the aliasing problem that appears naturally when reducing the samples on these axes.
Instead of changing the sampling mechanism, the authors in \cite{foged2016spherical} propose a new \ac{NFFFT} method with downsampling property during the acquisition process. A similar approach has been developed in  \cite{varela2020application} by using non-uniform Fourier transform to accommodate non-equiangular near-field acquisitions, in contrast to the original transformation method that employs conventional Fourier transforms with equiangular sampling points \cite{hansen1988spherical}.

Another strategy to address the long acquisition time is by employing Compressed Sensing (CS), which models the acquisition process as a linear system of equations and applies sparse recovery algorithms, e.g., \ac{BP}, to solve an underdetermined system of equations. This approach stems from the fact that, in most observations, the \ac{SMCs} are sparse or compressible, meaning that only a small amount of coefficients contains high power, as discussed in \cite{cornelius2015investigation, cornelius2016compressed, culotta2017radiationcenter, culotta2021dissertation}. 
%\textcolor{blue}{Therefore, we can assume that the underlying signal is sparse or compressible.} Since then, several extensions have been accomplished in this area \cite{culotta2018compressedsampling, fuchs2017fast, hofmann2019minimum, fuchs2018compressive}.

\textcolor{black}{
In \ac{CS} theory, if the sensing matrix satisfies certain conditions, for example \ac{RIP}, then it is guaranteed that sparse-recovery algorithms such as \ac{BP} yield a recovery error bounded by the measurement noise and model mismatch \cite{candes2005decoding,candes2006robust}}. 
%In particular, if the underlying signal is sparse, and the measurement is noiseless, one can completely recover the signal with enough measurements. Interestingly, the number of required measurements scales only logarithmically with the ambient dimension and linearly with sparsity order. For a detailed exposition of the \ac{CS} theory, we refer interested readers to \cite{foucart2013mathematical}.}
\textcolor{black}
{Random subgaussian matrices are known to satisfy \ac{RIP} with high probability and thereby have recovery guarantees. This is a considerable roadblock for the practical application of \ac{CS} in \ac{SNF}, since random sampling schemes cannot guarantee in any way that the mechanical movements required to scan them indeed reduce the acquisition time when compared to equiangular sampling schemes \cite{culotta2021dissertation}. Besides, it has been proven in \cite{bandeira2013certifying, tillmann2014computational} that verifying \ac{RIP} property for a given deterministic sensing matrices is an NP-hard problem. Therefore, the \ac{RIP} condition does not provide an adequate guideline for deterministic sensing matrix design}. Apart from \ac{RIP}, another approach to guaranteeing the recovery of sparse signals is the designing low-coherence sensing matrices. Despite providing a weaker reconstruction guarantee when compared to \ac{RIP}, the computation of the mutual coherence is computationally tractable, since it only consists of a dot product of adjacent columns of a sensing matrix. For this reason, designing a low-coherence sensing matrix is preferred in most applications, such as electromagnetic imaging \cite{obermeier2017sensing} and radar \cite{yu2011measurement}. In the mentioned examples, the implementation of \ac{CS} has been conducted by using the mutual coherence as a metric to numerically assess whether that the reconstruction algorithms yield a correct solution with fewer measurement points.

The challenge to construct a low-coherence sensing matrix in \ac{SNF} is that the multipole expansion of electromagnetic fields and antenna measurements requires specific functions, called spherical harmonics and Wigner D-functions, respectively. These functions follow certain polynomial structures, and their optimization is challenging. In this work, we present a method to optimize sensing matrices for \ac{SNF} in terms of their mutual coherence. 
%\ABCor{In contrast to our previous works where a certain parameter axes is fixed, e.g., on elevation $\theta$, in this work all variables on the parameter axes $(\theta, \phi, \chi)$ will be optimized.}
%{\color{red} To the best of our knowledge, this is the first work that discusses the optimization strategy of deterministic sensing matrix in the area of \ac{SNF}. } \todo[inline]{Think whether you want to put that there. Our previous works do exactly that, albeit with semi-deterministic matrices. In case we want to leave this in, it may be worth it to clarify that previous works (ours :) ) have done this for semi-deterministic matrices.}
%\textcolor{blue}{Arash: I agree. Our previous works do that. In some cases, part of the sampling patterns is fixed.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace*{-0.15cm}
\subsection{Related Works}
The construction of a sensing matrix from Wigner D-functions and their specific case, namely spherical harmonics, in the area of \ac{CS} has been  discussed in \cite{rauhut_sparse_2011,burq_weighted_2012,bangun2016sparse,bangun_sensing_2020}. However, these works emphasize more on the design of \ac{RIP} sensing matrices with random sampling and theoretical recovery guarantee using \ac{BP}. Although we have a bound on the minimum required number of measurements, in practice, this bound seems pessimistic, as discussed in \cite{hofmann2019minimum}, since the \ac{BP} algorithm is still able to numerically reconstruct the sparse coefficients even with fewer samples distributed in a spiral pattern. This investigation leads to the question of whether other types of deterministic sampling points can be designed to yield a higher recovery success, even if just numerically.

In \cite{bangun_coherence_2018,bangun_sensing_2020}, the authors aim to show that a specific sampling pattern, e.g., the equiangular sampling scheme, leads to the construction of a high coherence sensing matrix and fails to reconstruct the sparse signal which, in turn, excludes a construction of sensing matrices based on such a sampling strategy for \ac{CS} applications. Additionally, the authors derive an achievable coherence bound that can be used to design a low coherence sensing matrix for \ac{SNF} setting \cite{culotta2018compressedsampling}. %This bound can be achieved by fixing sampling points on the elevation axes $\theta \in [0,\pi]$ and optimizing only their azimuth coordinate $\phi \in [0, 2\pi)$ for \ac{SNF} setting \cite{culotta2018compressedsampling}. %These sampling points are not contrived since the implementation of such mechanism to construct a sensing matrix in an \ac{SNF} setting is achieved in . 
However, the drawback to this approach is that, while fixing a specific pattern on the elevation axes is advantageous for mechanical scanning systems, some degree of freedoms are lost in comparison to a full optimization on the whole spherical surface. 

%\todo[inline]{I commented some things here which I think are better deleted.}
%{\color{red}The optimization of the coherence of a sensing matrix is, in essence, the minimization of the maximum absolute value of the inner product in the column matrix. In \ac{SNF}, the problem is even trickier since we have to optimize the composite function, i.e., the angles of the Wigner D-functions or spherical harmonics.}
%In general, optimization of the coherence of a sensing matrix for \ac{SNF} is a non-convex problem because of the underlying Wigner D-functions and spherical harmonics, and a non-smooth optimization problem, due to the objective of minimizing the mutual coherence, i.e., the absolute value of the inner product of the columns of the matrix. 
\vspace*{-0.15cm}
\subsection{Summary of Contributions}
%In this article, we provide two algorithms to minimize the coherence of the sensing matrix for \ac{CS} applications in \ac{SNF}.
The main contributions of our paper are as follows:
\begin{itemize}
\item We propose a gradient-based method by smoothing the objective function to minimize the coherence in terms of $\ell_p$-norm. Thereby, we only have to set a large enough $p$ to approximate the maximum norm. %Numerically, we show that $p = 9$ is enough to get a good approximation. 
\item Besides, we also propose an \ac{ALM}-based proximal method. This approach provides an efficient strategy to decompose the original problem into subproblems. By using the proximal for the $\ell_{\infty}$-norm, we do not have to directly compute gradient or sub-gradient $\ell_{\infty}$-norm. 
\item We also provide numerical simulations to evaluate the coherence of a sensing matrix from both algorithms and compare them to the coherence of a sensing matrix constructed from well-known sampling patterns. %In addition, we also evaluate the performance of the sparse recovery for \ac{SMCs} in terms of phase transition diagrams. Furthermore, we also compare our optimized sensing matrices with the \ac{RIP} random sensing matrix for \ac{SNF}.
We  numerically show that our proposed sampling scheme outperform other well-known sampling patterns and deliver results similar to their random counterparts. 
\item At last, we apply optimized sensing matrices for experimental data and perform sparse \ac{SMCs} reconstruction, and use these to reconstruct the far-field pattern. Numerically, we show that by using optimized sensing matrices for \ac{CS} it is possible to reduce the number of samples to reconstruct an \ac{AUT}'s far-field pattern.
\end{itemize}

%\todo[inline]{I did not revise the part after the comment command}
\begin{comment}
\begin{itemize} 
\item Random sensing matrix for spherical harmonics, Wigner (Cite : Rauhut, Burq, Bangun Wigner, Bangun TSP). Explain why randomness nice in theory but not easy to implement in practice. Pessimistic recovery guarantee as shown in work Hoffman, et all
\item Related work to optimize sensing matrix (Cite, Elad, etc related to matrix optimization in CS)
\item Related work to optimize spherical harmonics, Wigner sensing matrix (Cite TSP Bangun, Cosme, AMTA, EUCAP paper)
\item Related to CS-SNF (Cited Hoffmann, etc see the citation from Fuchs etc, see who cited our paper and hoffman paper=
\end{itemize} 
\begin{itemize}
\item 1- In contraposition to using the "practical approach" of fixing theta to equidistant and taking chi = {0, pi/2} for the measurement, we make an optimization on the 3 angles at the same time using gradient descent.
\item 2- There is no theoretical bound but numerical results show a better (lower) coherence than for the other case.
\item 3- Reconstruction might work (will work?) better, at least theoretically.
\item 4- Some practical considerations can be added to see whether it is easily implementable and by which systems.
\item 5- The same approach as for EuCAP can be tested: after calculating the points, you can acquire further samples on the sampling path, they are for free and maybe reconstruction (surely) is improved.
\end{itemize}
fa
\textbf{Problems:}
\begin{itemize}
\item 1- Essentially we don't know if the sampling that we get in terms of (theta, phi) is scanable faster than the other one.
\item 2- You need to be able to change the polarization chi accurately.
\item 3- We don't know the bound (is there guarantee the coherence gets lower than for the fixed theta case, or is it just an empirical thing and maybe luck?)
\end{itemize}



\textbf{Introduction}
\begin{itemize}
\item Discuss spherical near-field antenna measurements, the inverse problem to estimate transmission coefficients and far-field transformation.
\item Classical approach to solve the inverse problem until recent approach using compressed sensing
\item Several approaches related to spherical near-field antenna measurement using compressed sensing
\end{itemize}
\end{comment}
 

==> Sections/opt_matrix.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Optimization of Sensing Matrices} \label{sec4_opt}
%The construction of a sensing matrix from Wigner D-functions depends on the sampling points acquired on the parameter axes, namely, elevation $\theta$, azimuth $\phi$, and polarization $\chi$.  
{Since the structure of a sensing matrix is restricted by certain properties of Wigner D-functions, the coherence optimization, therefore, boils down to finding optimal sampling points that yield a low coherence sensing matrix constructed from sampled Wigner D-functions.} The coherence of a sensing matrix from Wigner D-functions is given by 
\begin{equation} \label{coherence_Wigner}
\begin{aligned}
\mu  &= \underset{ 1 \leq r < q \leq L}{\text{max}} \card{g_{q,r} \left(\bs \theta,\bs \phi,\bs \chi \right)}\\   
\end{aligned},
\end{equation}
where $\card{g_{q,r} \left(\bs \theta,\bs \phi,\bs \chi \right)}$ is expressed as
\begin{equation}
    \small
 \card{\sum_{i = 1}^{K}\frac{\mathrm{D}^{n{(q)}}_{\mu{(q)},m{(q)}}(\theta_i,\phi_i,\chi_i)  \overline{\mathrm{D}^{n{(r)}}_{\mu{(r)},m{(r)}}(\theta_i,\phi_i,\chi_i)}}{\norm{\mathrm{D}^{n{(q)}}_{\mu{(q)},m{(q)}}(\boldsymbol\theta,\boldsymbol\phi,\boldsymbol\chi)}_2 \norm{\mathrm{D}^{n{(r)}}_{\mu{(r)},m{(r)}}(\boldsymbol\theta,\boldsymbol\phi,\boldsymbol\chi)}_2}}
 \label{eq:product}
\end{equation}
and the vector $\mathrm{D}^{n}_{\mu,m}(\boldsymbol\theta,\boldsymbol\phi,\boldsymbol\chi)$ is, in turn, 
\[
\small \mathrm{D}^{n}_{\mu,m}(\boldsymbol\theta,\boldsymbol\phi,\boldsymbol\chi)\defeq
\begin{pmatrix}
 \mathrm{D}^{n}_{\mu,m}(\theta_1,\phi_1,\chi_1),
 \hdots,
  \mathrm{D}^{n}_{\mu,m}(\theta_K,\phi_K,\chi_K)
\end{pmatrix}^T.
\]
The problem of optimizing the coherence of a sensing matrix from Wigner D-functions can be seen as finding the distribution of sampling points on $\theta \in [0, \pi]$ and $\phi, \chi \in [0, 2\pi)$ that minimizes \eqref{coherence_Wigner} as follows:

\begin{equation}
\begin{aligned}
\centering
& \underset{\bs \theta, \bs \phi, \bs \chi \in \R^K}{\text{min}}
& & \underset{ 1 \leq r < q \leq N}{\text{max}} \card{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}\\
%& \text{subject to}
%& & \theta_i \in [0,\pi]\quad \text{and} \quad \phi_i,\chi_i \in [0,2\pi) \quad  \\ &&&\text{for} \quad i \in [K]
\end{aligned}\quad.
\label{eq:Opt_General}
\end{equation}

This problem equals to solving the min-max optimization of a non-convex objective function.  In this work, we propose two approaches to tackle this optimization problem.

\subsection{Gradient-based $\ell_p$-norm}
The non-smoothness of the absolute value function poses a challenge in directly minimizing the coherence. However, %{\color{red}[IF YOU DON'T NAME THE PROPERTY DIRECTLY AFTERWARDS, SUCH AS "due to the whatever property of the...", THE SENTENCE DOES NOT MAKE MUCH SENSE. I WOULD DELETE THE RED PART]due to property of the $\ell_p$-norm,} 
%\todo[inline]{if the notation ends up in the appendix, reference to it here}
as presented in the notation in Section \ref{Sect:Appendix}, the $\ell_{\infty}$-norm can be approximated by the $\ell_p$-norm with a large enough $p$, as in
\begin{equation}
\begin{aligned}
\centering
&\underset{\bs \theta, \bs \phi, \bs \chi \in \R^K}{\text{min}}
& &\underset{p \rightarrow \infty}{\lim} \left(\underset{1 \leq r < q \leq N}{\sum} \card{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}^{p}\right)^{1/p}\\
%& \text{subject to} 
%& & \theta_i \in [0,\pi]\quad\text{and}\quad \phi_i,\chi_i \in [0,2\pi] \quad  \\ &&&\text{for} \quad i \in [K]
\end{aligned}\;\;.
\label{eq:Opt_Approx}
\end{equation}
%This strategy has been proposed in \cite{bangun2021tight}, but only to optimize the azimuth and polarization angles $\phi,\chi \in [0,2\pi)$ to achieve the lower bound derived from equispaced sampling points on $\theta \in [0,\pi]$. This strategy is obvious since the challenge in this approach is to optimize $\theta$ and for it, as opposed to variables $\phi$ and $\chi$, we have a more complex structure in terms of trigonometric functions and Jacobi polynomials, as expressed in \eqref{Wigner_d}. In this work, we adapt this optimization problem to optimize $\theta \in [0, \pi]$ and $\phi,\chi \in [0, 2\pi)$. We first show the derivative with respect to $\theta$ as follows

In contrast to the strategy in \cite{bangun2021tight} where only to optimize the azimuth and polarization angles $\phi,\chi \in [0,2\pi)$ to achieve the lower bound derived from equispaced sampling points on $\theta \in [0,\pi]$, the challenge when optimizing $\theta$, as opposed to variables $\phi$ and $\chi$, we have a more complex structure in terms of trigonometric functions and Jacobi polynomials, as expressed in \eqref{Wigner_d}. We first show the derivative with respect to $\theta$ as follows
\begin{equation} 
\footnotesize
\label{sec4_deriv}
\begin{aligned}
%\frac{1}{p}
\nabla_{\bs \theta} &\left(\underset{ 1 \leq r < q \leq L}{\sum} \card{{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}}^{p}\right)^{\frac{1}{p}} =\left(\underset{ 1 \leq r < q \leq L}{\sum} \card{{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}}^{p}\right)^{\frac{1 - p}{p}} \\& \times\left(\underset{ 1 \leq r < q \leq L}{\sum} \card{{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}}^{p - 1}\nabla_{\bs \theta} \card{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)} \right),\\
\end{aligned}
\end{equation} 
where $\nabla_{\bs \theta} \card{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}$ can be derived directly by taking the expression in \eqref{eq:product}, where the Wigner D-function is given by $\mathrm{D}_{\mu,m}^n(\theta,\phi,\chi) := e^{jm\phi} \mathrm{d}_{\mu,m}^n(\cos \theta) e^{j\mu\chi} $. The derivative with respect to $\bs \theta$ can be done by applying the product rule of derivatives, so that the derivative of Wigner d-functions, $\frac{\mathrm{d}}{\mathrm{d} \theta}\left(\mathrm{d}_{n}^{\mu,m}(\cos \theta)\right) $, can be expressed as
%\todo[inline]{Arya:Check again the derivatives!}
\begin{equation*}
\begin{aligned}
\small
 &\left({\frac{\xi \sin \theta}{2(1 - \cos \theta)}} - {\frac{\lambda \sin \theta}{2(1 + \cos \theta)}}  \right) \mathrm{d}_{n}^{\mu,m}(\cos \theta)  - {N_l}\sin \theta\,\omega \sqrt{\gamma}\\&\times \left(\frac{\xi + \lambda + \alpha + 1}{2}\right) \sin^{\xi}\left(\frac{\theta}{2} \right) \cos^{\lambda} \left( \frac{\theta}{2}\right)\times  P_{\alpha-1}^{\xi+1,\lambda + 1}(\cos \theta),
\end{aligned}
\end{equation*}
where the definition of $\mathrm{d}^{n}_{\mu,m}(\cos \theta)$  is given in \eqref{Wigner_d} and the chain rule is subsequently applied with respect to $\theta$, i.e., $\frac{\mathrm{d}}{\mathrm{d}\theta} f(\cos \theta) = -\sin \theta \frac{d}{d \cos \theta} f(\cos \theta) $. In addition, the $k$-th derivative of the Jacobi polynomials is given by
$$\small \frac{\mathrm{d}^k}{\mathrm{d} \cos^k \theta} { P_{\alpha}
^{\xi , \lambda} (\cos \theta)} = \frac{\Gamma(\xi + \lambda + \alpha + 1 + k)}{2^k \Gamma(\xi  + \lambda + \alpha + 1)} P_{\alpha - k}
^{\xi + k, \lambda + k} (\cos \theta)$$
where $\Gamma(x) = (x-1)!$. 

In addition, $\nabla_{\bs \phi}   \card{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}$ and $\nabla_{\bs \chi}   \card{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}$ are straightforward %\left(\underset{ 1 \leq r < q \leq L}{\sum} \card{{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}}^{p}\right)^{1/p} $  and $\nabla_{\bs \chi} \left(\underset{ 1 \leq r < q \leq L}{\sum} \card{{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}}^{p}\right)^{1/p} $ are trivial 
because we have trigonometric polynomials for orders $\mu, m$. Since the coherence should be evaluated in terms of the product of adjacent columns, the next step is to perform the product rule of derivative to complete the calculation of the gradient.

{Thereby, the variables $\bs \theta, \bs \phi$, and $\bs \chi$ can be iteratively updated by incorporating the gradient. For simplicity, we show the update for $\bs \theta$ at the $i$-th iteration as follows
\begin{equation}\label{eq:update_gd_theta}
\small
\bs{\theta}^{(i)} = \bs{\theta}^{(i-1)} - \eta \nabla_{\bs \theta} \left(\underset{ 1 \leq r < q \leq L}{\sum} \card{{g_{q,r}(\bs \theta^{(i-1)},\bs \phi^{(i-1)},\bs \chi^{(i-1)})}}^{p}\right)^{1/p} ,
\end{equation}
where the variable $\eta$ is the step size parameter. The same approach holds for $\bs \phi$ and $\bs \chi$. The summary of the procedure is given in Algorithm \ref{algo_gd}.} 


%\begin{comment}
\begin{algorithm}
    \caption{Gradient Descent of $\ell_p$-norm}\label{algo_gd}
    \begin{algorithmic}[1]
     
        \State \textbf{Initialization:} 
		\begin{itemize}
		\item Initial angles $\bs \theta^{(0)}, \bs \phi^{(0)}, \bs \chi^{(0)} \in \R^K$ uniformly random on interval $[0,\pi]$ and $[0,2\pi)$
		\item Step size $\eta \in \R$ and maximum iteration $T$
		\item Large enough $p$ for $\ell_{p}$-norm, initial coherence $\rho_0 = 1$.
 
		\end{itemize}
    \For{each iteration $i \in [T]$}  
    \State Update  $\bs \theta^{(i)}, \bs \phi^{(i)}$, and $\bs \chi^{(i)}$ as in \eqref{eq:update_gd_theta} 
    \If {$\underset{ 1 \leq r < q \leq N}{\text{max}} \card{g_{q,r}(\bs \theta^{(i)},\bs \phi^{(i)},\bs \chi^{(i)})} < \rho_{i-1}$ }
    	\State{$\rho_i = \underset{ 1 \leq r < q \leq N}{\text{max}} \card{g_{q,r}(\bs \theta^{(i)},\bs \phi^{(i)},\bs \chi^{(i)})}$}
   	\Else 
   		\State{$\rho_{i} = \rho_{i-1}$}
   %         \STATE \SEND{} Decrypt($ sk, V^{(2)}_t $)
	\EndIf
    \EndFor   
    \end{algorithmic}
  \end{algorithm} 
% \end{comment}
 

\subsection{\ac{ALM}-based algorithm} 

Instead of smoothing the $\ell_{\infty}$-norm through the $\ell_p$-norm for $p \in [2,\infty)$, we propose another approach by using the proximal method. In this case, we are not required to compute the gradient or subgradient directly. In the case of $\ell_{\infty}$-norm, its proximal operator can be written as the projection onto its dual norm, which is the $\ell_1$-norm \cite{parikh2014proximal}. Suppose we have a vector $\mbf x \in \R^L$, then the proximal operator of $\norm{\mbf x}_{\infty}$ is given by
\[
\text{prox}_{\norm{.}_\infty}\left(\mbf x\right) = \mbf x - \text{Proj}_{\norm{.}_1}\left( \mbf x \right).
\]
The projection onto the $\ell_1$-norm is well-studied, for instance, in \cite{duchi2008efficient} and can be directly implemented. 

The proximal method can be combined with the \ac{ALM} method to solve the optimization problem for minimizing the coherence of a sensing matrix.
%The advantage of using \ac{ALM} is that we can decompose the optimization problem into subproblems, hence, we can solve those subproblems separately and impose distributed optimization. This property is useful if we are dealing with a large scale optimization problem \cite{boyd2011distributed}.  
Let us assume we have set $\mcl{S} = \{\left(r,q\right) | 1 \leq r < q \leq L\}$, which represents the combinations of adjacent column matrices to evaluate the coherence with cardinality $\card{\mcl{S}} = J$. 
%We introduce a vector $$\mbf g \defeq [g_{q(1),r(1)}(\bs \theta,\bs \phi,\bs \chi), \hdots,g_{q(J),r(J)}(\bs \theta,\bs \phi,\bs \chi) ]^T \in \C^J,$$ where each element of the vector angles is restricted by
%$\theta_i \in [0,\pi]$ and $\phi_i,\chi_i \in [0,2\pi] \quad  \text{for} \quad i \in [K]$. 
Thereby, the optimization \eqref{eq:Opt_General} can be written as
\begin{equation}
\begin{aligned}
\centering
& \underset{\mbf{z} \in \C^J\atop\bs \theta, \bs \phi, \bs \chi \in \R^K}{\text{min}} \norm{\mbf z}_{\infty}
%& \text{subject to}
%& & \mbf z =  \mbf g
\text{subject to}
& & z_j = g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi), \quad {j \in [J]}
%&&& \theta_i \in [0,\pi], \phi_i,\chi_i \in [0,2\pi] \quad  \text{for} \quad i \in [K].
\end{aligned}
\label{eq:Opt_ALM}
\end{equation}
%Indeed, by introducing the auxiliary variable $\mbf z \in \C^J$, this problem is similar to the regularization of the $\ell_{\infty}$-norm.
We can write the scaled form of the augmented Lagrangian of the problem \eqref{eq:Opt_ALM} as 
$$
\small
\mcl{L}\left(\bs \theta, \bs \phi, \bs \chi, \mbf z, \mbf u \right) = \norm{\mbf z}_{\infty} + f\left(\bs \theta,\bs \phi,\bs \chi, \mbf z, \mbf u \ \right),
$$
where the constraint can be written as $f\left(\bs \theta,\bs \phi,\bs \chi, \mbf z, \mbf u\right) =  \sum_{j = 1}^J \frac{\tau}{2} \card{z_j - g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) + u_j}^2$.

Therefore, the procedure to optimize all variables in the augmented Lagrangian $\mcl{L}\left(\bs \theta, \bs \phi, \bs \chi, \mbf z, \mbf u \right)$ is now written as follows
\begin{align}
   & \mbf z^{\left(i \right)}= \underset{\mbf z}{\text{arg min}} \quad \mcl{L}\left(\bs \theta^{\left(i -1 \right)}, \bs \phi^{\left(i -1 \right)}, \bs \chi^{\left(i -1 \right)}, \mbf z, \mbf u^{\left(i -1 \right)} \right) \label{eq:update_z}\\
    &\bs \theta^{\left(i \right)},\bs \phi^{\left(i \right)},\bs \chi^{\left(i \right)}= \underset{\bs \theta,\bs \phi, \bs \chi}{\text{arg min}}  \quad \mcl{L}\left(\bs \theta , \bs \phi , \bs \chi , \mbf z^{\left(i -1 \right)}, \mbf u^{\left(i -1 \right)} \right)\label{eq:update_ang}\\
    &\small{\mbf u^{\left(i\right)} = \mbf u^{\left(i - 1\right)} + \tau \left(\mbf z^{\left(i\right) } - g_{q(j),r(j)}(\bs \theta^{\left(i \right)},\bs \phi^{\left(i \right)},\bs \chi^{\left(i \right)}) + \mbf u^{\left(i - 1\right)} \right)} \label{eq:update_u}
   %\left( \norm{\mbf z}_{\infty}  +  \sum_{j = 1}^J \frac{\tau}{2} \card{z_j - g_{q(j),r(j)}(\bs \theta^{\left(i -  1\right)},\bs \phi^{\left(i - 1\right)},\bs \chi^{\left(i -1 \right)}) + u_j^{\left(i - 1\right)}}^2\right)   
\end{align}
 
The complete \ac{ALM} algorithm can now be expressed as in Algorithm \ref{algo_ALM}.
\begin{algorithm} 
    \caption{\ac{ALM}-based algorithms}\label{algo_ALM}
    \begin{algorithmic}[1]
       
      \State \textbf{Initialization:} 
\begin{itemize}
    \item Initial angles $\bs \theta^{\left(0\right)} \bs \phi^{\left(0\right)}, \bs \chi^{\left(0\right)} \in \R^K$ uniformly random $[0,\pi]$ and $[0,2\pi)$
    \item Initial auxiliary variables $\mbf z^{\left(0\right)}, \mbf u^{\left(0\right)} \in \C^J$
    \item Number of iteration $T$, scaling parameters $\tau$, initial coherence $\rho_0 = 1$
   
    \end{itemize}
     \For {each iteration $i \in [T]$ }
    \State Update $\mbf z$ from \eqref{eq:update_z}
    \State Update  $\bs \theta,\bs \phi,\bs \chi$  from \eqref{eq:update_ang}
    \State Update $\mbf u$ from \eqref{eq:update_u}
      \If {$\underset{ 1 \leq r < q \leq N}{\text{max}} \card{g_{q,r}(\bs \theta^{(i)},\bs \phi^{(i)},\bs \chi^{(i)})} < \rho_{i-1}$ }
    	\State{$\rho_i = \underset{ 1 \leq r < q \leq N}{\text{max}} \card{g_{q,r}(\bs \theta^{(i)},\bs \phi^{(i)},\bs \chi^{(i)})}$}
   	\Else 
   		\State{$\rho_{i} = \rho_{i-1}$}
   %         \STATE \SEND{} Decrypt($ sk, V^{(2)}_t $)
	\EndIf
    \EndFor   
    \end{algorithmic}
\end{algorithm} 
%It should be noted again that, in general, \ac{ALM} is an optimization approach that consists of several subproblems. In Algorithm \ref{algo_ALM}, we have to solve an optimization with respect to the auxiliary variable $\mbf z$ and angles $\theta,\phi,\chi$, as described in  \eqref{eq:update_z},\eqref{eq:update_ang}, and \eqref{eq:update_u}. In what follows, we will describe the algorithms to address those subproblems. 
Equation \eqref{eq:proximal} presents the update procedure for the proximal $\ell_{\infty}$-norm as in  \eqref{eq:update_z}. 
%The advantage of the proximal method is that, after computing the update for smooth objective functions, in this case, the $\ell_2$-norm constraints, we can incorporate this result into the proximal method. 
\begin{equation}
 \begin{aligned}
   & \mbf{\hat z}  = \mbf z^{\left(i-1 \right)} - \eta \nabla_{\mbf z } f\left(\theta^{\left(i -1 \right)}, \bs \phi^{\left(i -1 \right)}, \bs \chi^{\left(i -1 \right)}, \mbf z, \mbf u^{\left(i-1\right)}\right)\\
%\left(\sum_{j = 1}^J \frac{\tau}{2} \card{z_j - g_{q(j),r(j)}\left(\theta^{\left(i -1 \right)}, \bs \phi^{\left(i -1 \right)}, \bs \chi^{\left(i -1 \right)}\right) + u_j^{\left(i-1\right)}}^2\right)    \\
&\mbf z^{\left(i\right)} =  \mbf{\hat z} - \lambda \eta \text{Proj}_{\norm{.}_1}\left( \frac{\mbf{\hat z} }{\eta \lambda} \right)\label{eq:proximal}, 
\end{aligned}   
\end{equation}
where  $\lambda$ is the regularization parameter.
\begin{comment}
\begin{algorithm} 
    \caption{Proximal to update $\mbf z$}\label{algo_proximal}
    \begin{algorithmic}[1]  
      \State \textbf{Initialization:}
      \begin{itemize}
      \item Current vector  $\mbf z \in \R^J$$g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) \quad \text{for} \quad {j \in [J]}$,
      \item Current scaled Lagrange multiplier: $\mbf u \in \R^J$
      \item Reqularization $\lambda, \tau$, step size $\eta$
	  \end{itemize}       
     %\FOR    $i \in [T]$  
     \State Update $\ell_2$-norm constraint: $\mbf z_{temp} = \mbf z - \eta \nabla_{\mbf z } 
\left(\sum_{j = 1}^J \frac{\tau}{2} \card{z_j - g_{q(j),r(j)}\left(\bs \theta,\bs \phi,\bs \chi\right) + u_j}^2\right)    
     $
     
     \State Proximal $\ell_{\infty}$-norm for $\mbf z$: $\text{prox}_{\norm{.}_\infty}\left(\mbf z_{temp}\right)
      = \mbf z_{temp} - \eta \lambda \text{Proj}_{\norm{.}_1}\left( \frac{z_{temp}}{\eta \lambda} \right)$

   %  \end{equation*} $
    %\ENDFOR   
    \end{algorithmic}
\end{algorithm} 
\end{comment}
Additionally, we also provide the update for angles $\bs \theta, \bs \phi, \bs \chi$ in \eqref{eq:update_angles} to solve \eqref{eq:update_ang}. 
%In this case, the gradient with respect to different angles should be calculated, which is already derived in the previous section when performing a gradient-based algorithm. 
For simplicity,  we only write the update $\bs \theta$. The update $\bs \phi$ and $\bs \chi$ can be adapted by changing the gradient index.

\begin{equation}
    \begin{aligned}
    \label{eq:update_angles}
     \bs \theta^{\left(i\right)} = \bs\theta^{\left(i-1\right)} - &\eta \nabla_{\bs \theta } f\left(\theta^{\left(i -1 \right)}, \bs \phi^{\left(i -1 \right)}, \bs \chi^{\left(i -1 \right)}, \mbf z^{\left( i\right)}, \mbf u^{\left(i-1\right)}\right) \\
     %\left(\sum_{j = 1}^J \tau \card{z_j - g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) + u_j}\right) \\
     &\times\nabla_{\bs \theta } \left( g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) \right)\\
          %\bs \phi^{\left(i\right)} = \bs\phi^{\left(i-1\right)} - \eta &\nabla_{\bs \phi } f\left(\theta^{\left(i -1 \right)}, \bs \phi^{\left(i -1 \right)}, \bs \chi^{\left(i -1 \right)}, \mbf z^{\left( i\right)}, \mbf u^{\left(i-1\right)}\right) \\
     %\left(\sum_{j = 1}^J \tau \card{z_j - g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) + u_j}\right) \\
     %&\times\nabla_{\bs \phi } \left( g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) \right)\\
     %\bs \chi^{\left(i\right)} = \bs\chi^{\left(i-1\right)} - \eta &\nabla_{\bs \chi } f\left(\theta^{\left(i -1 \right)}, \bs \phi^{\left(i -1 \right)}, \bs \chi^{\left(i -1 \right)}, \mbf z^{\left( i\right)}, \mbf u^{\left(i-1\right)}\right) \\
     %\left(\sum_{j = 1}^J \tau \card{z_j - g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) + u_j}\right) \\
     %&\times\nabla_{\bs \chi } \left( g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) \right)
     \end{aligned}
\end{equation}
\begin{comment}
\begin{algorithm} 
    \caption{Update for $\bs \theta, \bs \phi, \bs \chi \in \R^K$}\label{algo_update_angles}
    \begin{algorithmic}[1]
      \State \textbf{Initialization:}  
      \begin{itemize}
      \item Current angles $\bs \theta, \bs \phi, \bs \chi$
      \item Current scaled Lagrange multiplier: $\mbf u \in \R^J$
      \item Regularization $\tau$, step size $\eta$
      \item Current vector : $g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) \quad \text{for} \quad  {j \in [J]}$, $\mbf z \in \R^J$
      \end{itemize}
     %\FOR    $i \in [T]$ 
    \State Update $\bs \theta$: 
    \begin{align*} \bs \theta - \eta &\left(\sum_{j = 1}^J \tau \card{z_j - g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) + u_j}\right) \\\times\nabla_{\bs \theta } \left( g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) \right)\end{align*}
    \State Update $\bs \phi$: $\bs \phi - \eta \left(\sum_{j = 1}^J \tau \card{z_j - g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) + u_j}\right) \nabla_{\bs \phi } \left( g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) \right)$ 
    \State Update $\bs \chi$: $\bs \chi - \eta \left(\sum_{j = 1}^J \tau \card{z_j - g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) + u_j}\right) \nabla_{\bs \chi } \left( g_{q(j),r(j)}(\bs \theta,\bs \phi,\bs \chi) \right)$ 
    %\ENDFOR   
    \end{algorithmic}
\end{algorithm} 
\end{comment}
%\ABCor{It can be seen in Algorithm \ref{algo_gd} and Algorithm \ref{algo_ALM} that step size $\eta$ is an important variable to guarantee the optimality of the algorithm. In this paper, we can implement a backtracking line search \cite{armijo1966minimization}\cite[Ch.3]{nocedal2006numerical} to determine the step size $\eta$. It should be noted that after updating each variable we should evaluate again the backtracking line search to get new step size parameter $\theta$.}
For both cases, gradient-based and \ac{ALM}-based, the optimization problem for Wigner D-function can be easily tailored for the spherical harmonics case by setting degree $\mu = 0$ in \eqref{coherence_Wigner} \cite{bangun2020dissertation, culotta2021dissertation}.  
\begin{comment}
 
\begin{equation*}
\begin{aligned}
 &\frac{\mathrm{Re}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right] \nabla_{\bs \theta}\left(\mathrm{Re}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]\right)  }{ \sqrt{\left(\mathrm{Re}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]\right)^2 + \left(\mathrm{Im}\left[g_{q,r}(\bs \theta,\bs \phi,\bs \chi)\right] \right)^2}} + \\ &\frac{\mathrm{Im}\left[g_{q,r}(\bs \theta,\bs \phi,\bs \chi)\right] \nabla_{\bs \theta}\left(\mathrm{Im}\left[g_{q,r}(\bs \theta,\bs \phi,\bs \chi)\right] \right)}{\sqrt{\left(\mathrm{Re}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]\right)^2 + \left(\mathrm{Im}\left[g_{q,r}(\bs \theta,\bs \phi,\bs \chi)\right] \right)^2}}
\end{aligned}    
\end{equation*}
%&= \frac{1}{p}\left(\underset{ 1 \leq r < q \leq L}{\sum} \card{{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}}^{p}\right)^{\frac{1}{p} - 1}  \left(\underset{ 1 \leq r < q \leq L}{\sum} p \card{{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}}^{p - 1}\right)\\
%&\quad \times \frac{1}{2}\left[ \left(\mathrm{Re}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]\right)^2 + \left(\mathrm{Im}\left[g_{q,r}(\bs \theta,\bs \phi,\bs \chi)\right] \right)^2 \right]^{-\frac{1}{2}} \\
%&\quad \times \left(\nabla_{\bs \theta} \left(\mathrm{Re}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]\right)^2 + \nabla_{\bs \theta} \left(\mathrm{Im}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]\right)^2 \right) \\
%& =  \left(\underset{ 1 \leq r < q \leq L}{\sum} \card{{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}}^{p}\right)^{\frac{1}{p} - 1}  \left(\underset{ 1 \leq r < q \leq L}{\sum}  \card{{g_{q,r}(\bs \theta,\bs \phi,\bs \chi)}}^{p - 2}\right)\\
%&\quad \times \mathrm{Re}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]\nabla_{\bs \theta} \left(\mathrm{Re}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]\right) \\
%&\quad +\mathrm{Im}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]\nabla_{\bs \theta} \left(\mathrm{Im}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]\right) .

Equation \eqref{sec4_deriv} holds in general if we also want to derive with respect to $\phi,\chi$. From \eqref{coherence_Wigner}, we have expression of $g_{q,r}(\bs \theta,\bs \phi,\bs \chi)$. Hence, we have $$\nabla_{\theta_j} \mathrm{Re}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right] = \frac{\nabla_{\theta_j}\left(\mathrm{d}^{n{(q)}}_{\mu{(q)},m{(q)}}(\cos \theta_j)  \mathrm{d}^{n{(r)}}_{\mu{(r)},m{(r)}}(\cos \theta_j) \right) \cos\left[(m(q) - m(r))\phi_j + (\mu(q) - \mu(r)) \chi_j\right]}{\norm{\mathrm{D}^{n{(q)}}_{\mu{(q)},m{(q)}}(\boldsymbol\theta,\boldsymbol\phi,\boldsymbol\chi)}_2 \norm{\mathrm{D}^{n{(r)}}_{\mu{(r)},m{(r)}}(\boldsymbol\theta,\boldsymbol\phi,\boldsymbol\chi)}_2}.$$ It can be seen that the result for $\nabla_{\theta_j} \mathrm{Im}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]$ is straightforward by changing cosine factor into sine and $\nabla_{\theta_j}\left(\mathrm{d}^{n{(q)}}_{\mu{(q)},m{(q)}}(\cos \theta_j)  \mathrm{d}^{n{(r)}}_{\mu{(r)},m{(r)}}(\cos \theta_j) \right)$ can be calculated by using product rule. In addition, using \eqref{Wigner_d},  derivative of $\mathrm{d}^{n}_{\mu,m}(\cos \theta)$ can be expressed as

\begin{equation*}
\small
\begin{aligned}
\frac{\mathrm{d}}{\mathrm{d} \theta} \mathrm{d}_{n}^{\mu,m}(\cos \theta) &= \left( \frac{\lambda \sin^2 \theta}{2(1 + \cos \theta)} - \frac{\xi \sin^2 \theta}{2(1 - \cos \theta)}  \right) \mathrm{d}_{n}^{\mu,m}(\cos \theta) - \sin \theta\\
&\times \omega \sqrt{\gamma}\left(\frac{\xi + \lambda + \alpha + 1}{2}\right) \sin^{\xi}\left(\frac{\theta}{2} \right) \cos^{\lambda} \left( \frac{\theta}{2}\right)   P_{\alpha-1}^{\xi+1,\lambda + 1}(\cos \theta),
\end{aligned}
\end{equation*}
where the definition of $\mathrm{d}^{n}_{\mu,m}(\cos \theta)$  is given in \eqref{Wigner_d} and apply chain rule with respect to $\theta$, i.e., $\frac{d}{d\theta} f(\cos \theta) = -\sin \theta \frac{d}{d \cos \theta} f(\cos \theta) $. In addition, $k$-derivative of Jacobi polynomial is given by [] $$\frac{d^k}{d \cos^k \theta} = \frac{\Gamma(\xi + \lambda + \alpha + 1 + k)}{2^k \Gamma(\xi  + \lambda + \alpha + 1)} P_{\alpha - k}
^{\xi + k, \lambda + k} (\cos \theta),$$
where $\Gamma(x) = (x-1)!$.

The gradient for $\phi$, $\nabla_{\phi_j} \mathrm{Re}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]$, can be written as
$$ \frac{\mathrm{d}^{n{(q)}}_{\mu{(q)},m{(q)}}(\cos \theta_j)  \mathrm{d}^{n{(r)}}_{\mu{(r)},m{(r)}}(\cos \theta_j) \nabla_{\phi_j}\left(\cos\left[(m(q) - m(r))\phi_j + (\mu(q) - \mu(r)) \chi_j\right]\right)}{\norm{\mathrm{D}^{n{(q)}}_{\mu{(q)},m{(q)}}(\boldsymbol\theta,\boldsymbol\phi,\boldsymbol\chi)}_2 \norm{\mathrm{D}^{n{(r)}}_{\mu{(r)},m{(r)}}(\boldsymbol\theta,\boldsymbol\phi,\boldsymbol\chi)}_2},$$
where $\nabla_{\phi_j}\left(\cos\left[(m(q) - m(r))\phi_j + (\mu(q) - \mu(r)) \chi_j\right]\right)$ can be written as
$$-(m(q) - m(r))\sin\left[(m(q) - m(r))\phi_j + (\mu(q) - \mu(r)) \chi_j\right].$$ 
One can get the same result for $\nabla_{\chi_j} \mathrm{Re}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]$ by changing the factor $-(m(q) - m(r))$ with $-(\mu(q) - \mu(r))$. Similar approach can be used to derive $\nabla_{\phi_j} \mathrm{Im}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]$ and  $\nabla_{\chi_j} \mathrm{Im}\left[ g_{q,r}(\bs \theta,\bs \phi,\bs \chi) \right]$. The only caveat is that instead of having factor negative sine, we arrive at factor positive cosine because the property of derivation for trigonometric functions. 
\end{comment}

==> Sections/snf.tex <==
\section{Spherical Near-Field Measurements}\label{sec3_snf}
%In this section, the short overview of spherical near-field measurement will be discussed. 
{\color{black}Electromagnetic fields can be modelled as} a superposition of harmonic functions and have, therefore, a periodic structure. Specifically, the radiated fields that are acquired by a probe antenna can be expanded by orthogonal basis functions that solve Maxwell's equations \cite[Eq 4.43]{hansen1988spherical}. We can express the relation as follows:
%\todo[inline]{I have changed the constant $v$ right before the SMCs to $u$ to avoid confusion with the summation for $\mu$}
\begin{equation}
\footnotesize
w(r,\theta,\phi,\chi)= \sum \limits_{\mu=-v_\text{max}}^{v_\text{max}}\sum\limits_{s=1}^2\sum\limits_{n=1}^N\sum\limits_{m=-n}^n \mathrm{D}_{\mu,m}^n(\theta,\phi,\chi)  uT_{smn} P_{s\mu n} (kr),
\label{sec3_trans_eq}
\end{equation} 
where $\mathrm{D}_{\mu,m}^n(\theta,\phi,\chi) := e^{jm\phi} \mathrm{d}_{\mu,m}^n(\cos \theta) e^{j\mu\chi} $ are the Wigner D-functions of degree $n$ and orders $\mu,m$. Mathematically, these functions act as basis functions in the three-dimensional rotation space to represent electromagnetic fields. The function $\mathrm{d}_{\mu,m}^n(\cos \theta)$ represents the Wigner d-functions, defined by
\begin{equation} \label{Wigner_d}
\mathrm{d}_{\mu,m}^{n}(\cos \theta)\defeq \omega \sqrt{\gamma} \sin^{\xi} \bigg(\frac{\theta}{2}\bigg)\cos^{\lambda}\bigg(\frac{\theta}{2}\bigg) P_{\alpha}^{(\xi,\lambda)}(\cos \theta),
\end{equation}
where $\gamma = \frac{\alpha!(\alpha + \xi + \lambda)!}{(\alpha+\xi)!(\alpha+\lambda)!}$, $\xi=\card{m - \mu}$, $\lambda=\card{m + \mu}$, $\alpha= n -\big(\frac{\xi+\lambda}{2}\big)$. For $\mu \geq m $ the value $ \omega = 1$ otherwise $(-1)^{\mu-m}$.
%\begin{equation*}
% \omega= \begin{cases} 
%        1  & \text{if } \mu \geq m  \\
%        (-1)^{\mu-m} & \text{if } \mu < m 
%          \end{cases}.
%\end{equation*}
The function $P_{\alpha}^{(\xi,\lambda)}$ represents the Jacobi polynomials. The Wigner D-functions bear a strong resemblance with a set of orthogonal basis functions on the sphere: the spherical harmonics. The relation between these basis functions can be derived by considering the order $\mu = 0$:
\begin{equation}
\mathrm{D}_{0,m}^n(\theta,\phi,\chi) =  (-1)^m \sqrt{\frac{4\pi}{2n + 1}} \Y{n}{m}(\theta, \phi),
\label{eq.sh_wign}
\end{equation}
where the spherical harmonics $\Y{n}{m}(\theta, \phi)$ can be expressed as the product of associated Legendre and trigonometric polynomials
$$\Y{n}{m}(\theta,\phi) = \sqrt{\frac{2n + 1}{4\pi}\frac{(n-m)!}{(n + m )!}} P_n^m(\cos \theta) e^{im\theta}.$$

Classically, it is considered that, after a certain degree $n = N$, the contribution of higher modes to the total power of the expansion is limited. The truncation constant applied is typically calculated as $N = k r_{min} + N_0$, where $k=\nicefrac{2\pi}{\lambda}$ is the wavenumber, $r_{min}$ is the minimum radius of the sphere that encloses the \ac{AUT}, and $N_0$ is a constant for accuracy, whereby $N_0 = 10$ is supported in the literature \cite{hansen1988spherical}. Additionally, {\color{black}$v_\text{max}$ depends on the distance the probe antenna is being considered at, i.e., $v_\text{max} = N$ generally, since its modes are displaced with respect to the center of the coordinate system of the measurement.} %\todo[inline]{I tried to salvage the explanation related to the indices of the probe and to simplify it so that it is consistent with the used equations, but it actually makes sense from a measurement perspective.} 
In \eqref{sec3_trans_eq}, $u$ is the input signal to the \ac{AUT} and $w(r, \theta, \phi, \chi)$ is the radiated field acquired by a given measurement probe at a distance $r$, with elevation $\theta \in [0,\pi]$ and with azimuth angle $\phi \in [0, 2\pi)$. The response of the probe itself, i.e., the radiation pattern of the probe itself, affects the measured signal as well. The probe response constants $P_{s\mu n} (kr)$ describe this behavior in the acquisition process. Additionally, another factor comes into play: the polarization characteristics of both \ac{AUT} and probe. To measure it, the polarization angle $\chi \in [0, 2\pi)$ is added. Fig.~\ref{fig:SNF_Setting} shows the described measurement geometry.
\begin{figure}[!htb] 
\centering
\inputTikZ{0.6}{Figure/CouplingGeometry_TAP.tex}
%\inputTikZ{0.7}{Figure/PositionAUTandSMC_Muster.tex}
\caption{Measurement settings for \ac{SNF}}
\label{fig:SNF_Setting}
\end{figure}
The transmission coefficients $T_{smn}$ can be decomposed into transverse electric and transverse magnetic coefficients, described by $T_{1mn}$ and $T_{2mn}$, respectively, and are useful to determine properties of the \ac{AUT} in the far-field region. The objective of \ac{SNF} measurements is, ultimately, to solve the inverse problem that derives the transmission coefficients $T_{smn}$ from near-field measurements by solving the linear equations resulting from \eqref{sec3_trans_eq}. Once the $T_{smn}$ are known, the \ac{AUT}'s far-field characteristic can be easily computed by solving \eqref{sec3_trans_eq} for $r\to\infty$, which represents the theoretical far field.
\vspace*{-0.15cm}
\subsection{General Case} \label{Sec:General}
Suppose we acquire $K$ samples of radiated fields on the unit sphere $w(\theta_i,\phi_i. \chi_i)$ for $i \in [K]$. {We consider the general case with $v_\text{max} = n$}. %\todo[inline]{This is wrong. The reason why $N = v_{max}$ has nothing to do with its radius: the reason is that the modes of the probe are considered in the framework of the measurement, i.e., the center of the reference system is the same as the center of the AUT. So the coefficients of the probe are displaced, which means that it is "as if" the radius were larger. These translation coefficients are included in $P_{s\mu n}(kr)$, so I will have to include this in the following equation as well.}
Thereby, we can rewrite \eqref{sec3_trans_eq} into
\begin{equation}
\begin{aligned}
 %w(\theta_i,\phi_i,\chi_i) &= 
 \sum\limits_{n = 1}^N \sum\limits_{m = -n}^n \sum\limits_{\mu = -n}^n \mathrm{D}_{\mu m}^n(\theta_i,\phi_i,\chi_i)\left(c_{1mn\mu}  + c_{2mn\mu} \right),
\label{sec3_expand}
\end{aligned}
\end{equation}
where we write $c_{smn\mu}= uT_{snm}P_{s\mu n}(k)$ as the product between transmission coefficients and the probe response constants with input signal $u$. We can then represent equation \eqref{sec3_expand} in matrix and vector form as in \eqref{eq:linear_meas},
%\begin{equation}
%\mbf{y} = \mbf{A} \mbf{x},
%\end{equation}
%where the spherical near-field samples and element-wise product of the transmission coefficients and the probe are given by
%\[
%\vec{y}=\begin{pmatrix}
%  y_1\\
%  \vdots\\
%  y_K
%\end{pmatrix},
%\vec{x}=\begin{pmatrix}
%  x_1\\
%  \vdots\\
%  x_L
%\end{pmatrix}.
%\]
where the elements of vector $\mbf{y} \in \C^{K}$ and coefficients $\mbf x \in \C^{L}$ are given by $y_i = w(\theta_i,\phi_i,\chi_i)\quad \text{for}\quad i \in [K]$ and $x_q~=~\left(c_{1 m(q) n(q) \mu(q)}  + c_{2 m(q) n(q) \mu(q)} \right) \quad \text{for}\quad q \in [L]$,
respectively. The sensing matrix $\mat{A} \in \C^{K \times L}$ is given by 
\begin{equation}
\small
\mat{A}=
\begin{pmatrix}
  \mathrm{D}^{1}_{-1,-1}(\theta_1,\phi_1,\chi_1)&\dots& \mathrm{D}^{B-1}_{B-1,B-1}(\theta_1,\phi_1,\chi_1) \\
  \vdots\\
  \mathrm{D}^{1}_{-1,-1}(\theta_K,\phi_K,\chi_K)&\dots& \mathrm{D}^{B-1}_{B-1,B-1}(\theta_K,\phi_K,\chi_K)
\end{pmatrix},
\label{sec_3.sensingmatrix}
\end{equation}
where columns of this matrix consist of $K$ different samples of Wigner D-functions. For clarity, we can write the elements of a matrix $\mat{A} \in \C^{K \times L}$  as
\begin{equation}
A_{iq} = \mathrm{D}_{\mu(q) m(q)}^{n(q)}(\theta_i,\phi_i,\chi_i),
\end{equation}
where the column dimension $L = \frac{4N^3 + 12N^2 + 11N}{3}$, which is determined by a combination of degree and orders $n(q),m(q),\mu(q)$, respectively.  
\vspace*{-0.15cm}
\subsection{Specific Case}\label{Sec:Specific}   
As discussed in \cite{hansen1988spherical, wacker1975non}, assuming only the $\mu = \pm 1$ modes of the probe contribute significantly to the measurement is enough for most cases and considerably reduces the computational complexity of the problem. This assumption is valid for most linearly polarized probes. %{\color{red}[DELETE]it is enough to use a linearly polarized probe to carry out the acquisition process, i.e., when mode  $\mu = \pm 1$. [EXPLANATION] It doesn't really have much to do with the polarization. True, a well-aligned linearly polarized probe only has odd $\mu$ modes, but not only $\pm1$ ones.} 
%Following this approach, we can rewrite \eqref{sec3_expand} into 
%\begin{equation}
%\begin{aligned}
%  %w(\theta_i,\phi_i,\chi_i)=&
%  \sum\limits_{n = 1}^N \sum\limits_{m = -n}^n  &\mathrm{D}_{1 m}^n(\theta_i,\phi_i,\chi_i)\left(c_{1mn1}  + c_{2mn1} \right) +   \\\sum\limits_{n = 1}^N \sum\limits_{m = -n}^n&\mathrm{D}^n_{-1 m}(\theta_i,\phi_i,\chi_i) \left(c_{1mn-1}  + c_{2mn-1} \right) ,
%  \label{eq:spec_case}
%\end{aligned}
%\end{equation}
%for $i \in [K]$. 
%Let us focus on the first term in \eqref{sec3_expand}, we can write 
%\begin{equation}
% \sum\limits_{n=1}^N\sum\limits_{m=-n}^n \mathrm{D}^n_{1 m}(\theta_p,\phi_p,\chi_p)c_{1mn1}(kA) +\sum\limits_{n=1}^N\sum\limits_{m=-n}^n \mathrm{D}^n_{1 m}(\theta_p,\phi_p,\chi_p)c_{2mn1}(kA)
%\label{sec3_expand2}
%\end{equation}
%Now expand both formula for $s=1,2$ so the equation can be written separately:
%\begin{equation}
%X=\sum\limits_{n=1}^N\sum\limits_{m=-n}^n \psi^n_{1 m}(\theta,\phi,\chi)c_{1mn1}(kA)+\sum\limits_{n=1}^N\sum\limits_{m=-n}^n \psi^n_{1 m}(\theta,\phi,\chi)c_{2mn1}(kA)
%\label{eq:no5_matrix_expandA}
%\end{equation}
%\begin{equation}
%Y=\sum\limits_{n=1}^N\sum\limits_{m=-n}^n \psi^n_{-1 m}(\theta,\phi,\chi)c_{1mn-1}(kA)+\sum\limits_{n=1}^N\sum\limits_{m=-n}^n \psi^n_{-1 m}(\theta,\phi,\chi)c_{2mn-1}(kA).
%\label{eq:no6_matrix_expandB}
%\end{equation}
Elaborating further, and as discussed in \cite[Eq 4.99]{hansen1988spherical}, a linearly polarized probe has symmetric and anti-symmetric properties for each transverse electric $s = 1$ and magnetic $s = 2$ mode, as expressed by $ c_{smn(\mu=-1)} =  c_{smn(\mu=1)}
$ for $s = 1$ and $c_{smn(\mu=-1)} =  -c_{smn(\mu=1)} $ for $s = 2$.
%\[
% c_{smn(\mu=-1)} =
%  \begin{cases}
%   c_{smn(\mu=1)} & %\text{if } s=1 \\
%   -c_{smn(\mu=1)}     & \text{if } s=2
%  \end{cases}\;.
%\]
Therefore, we can treat %\eqref{eq:spec_case} 
\eqref{sec3_expand}
 as the superposition of two expansions and rewrite it into
\begin{equation}
\begin{aligned}
%w(\theta_i,\phi_i,\chi_i) =  
&\sum\limits_{n = 1}^N \sum\limits_{m = -n}^n \bigg(\mathrm{D}_{1 m}^n(\theta_i,\phi_i,\chi_i) +\mathrm{D}^n_{-1 m}(\theta_i,\phi_i,\chi_i) \bigg) c_{1mn1}  + \\
&\sum\limits_{n = 1}^N\sum\limits_{m = -n}^n \bigg(\mathrm{D}_{1 m}^n(\theta_i,\phi_i,\chi_i) -  \mathrm{D}^n_{-1 m}(\theta_i,\phi_i,\chi_i) \bigg) c_{2mn1}
\label{sec3_expand2}
\end{aligned}
\end{equation}
or, equivalently, in matrix form as 
\begin{equation}
\begin{aligned}
\mathbf{y} = \left[\begin{array}{c} \mathbf{A_1} \quad \mathbf{A_2} \end{array}\right]\left[\begin{array}{c} \mathbf{x_1}\\ \mathbf{x_2}  \end{array}\right], 
\end{aligned}
\end{equation}
where the elements of matrices $\mbf{A_1},\mbf{A_2} \in \C^{K \times L}$ are, in turn, given by
\begin{equation}
A_{iq}^1 =  \mathrm{D}_{1 m(q)}^{n(q)}(\theta_i,\phi_i,\chi_i) + \mathrm{D}_{-1 m(q)}^{n(q)}(\theta_i,\phi_i,\chi_i),
\end{equation}
\vspace*{-0.5cm}
\begin{equation}
A_{iq}^2 = \mathrm{D}_{\mu(q) m(q)}^{n(q)}(\theta_i,\phi_i,\chi_i) - \mathrm{D}_{\mu(q) m(q)}^{n(q)}(\theta_i,\phi_i,\chi_i),
\end{equation}
and for each matrix we have column dimension $L$. Similarly, the transmission coefficients can be expressed as element vectors $\mbf{x}_1,\mbf{x}_2 \in \C^L$ and are given by $x^1_{q} = c_{1m(q)n(q)1}$ and $x^2_{q} = c_{2m(q)n(q)1}$ for a combination degree $m(q)$ and order $n(q)$, respectively. %Since we have constructed a system of linear equations for \ac{SNF} and sensing matrices, we can incorporate the \ac{BP} program to estimate the sparse \ac{SMCs} from fewer \ac{SNF} samples. In what follows, we discuss the strategy to optimize the sensing matrices in terms of coherence to make sure that the \ac{BP} program delivers the optimal solution.

